The NANOGrav 15-year Data Set: Search for Gravitational Wave Memory

We present the results of a search for nonlinear gravitational wave memory in the NANOGrav 15-year data set. We find no significant evidence for memory signals in the dataset, with a maximum Bayes factor of 3.1 in favor of a model including memory. We therefore place upper limits on the strain of potential gravitational wave memory events as a function of sky location and observing epoch. We find upper limits that are not always more constraining than previous NANOGrav results. We show that it is likely due to the increase in common red noise between the 12.5-year and 15-year NANOGrav datasets.

==> acksBWM15.tex <==
L.B.\ acknowledges support from the National Science Foundation under award AST-1909933 and from the Research Corporation for Science Advancement under Cottrell Scholar Award No.\ 27553.
P.R.B.\ is supported by the Science and Technology Facilities Council, grant number ST/W000946/1.
S.B.\ gratefully acknowledges the support of a Sloan Fellowship, and the support of NSF under award \#1815664.
The work of R.B., N.La., X.S., J.P.S., J.T., and D.W.\ is partly supported by the George and Hannah Bolinger Memorial Fund in the College of Science at Oregon State University.
M.C., P.P., and S.R.T.\ acknowledge support from NSF AST-2007993.
M.C.\ was supported by the Vanderbilt Initiative in Data Intensive Astrophysics (VIDA) Fellowship.
Support for this work was provided by the NSF through the Grote Reber Fellowship Program administered by Associated Universities, Inc./National Radio Astronomy Observatory.
Pulsar research at UBC is supported by an NSERC Discovery Grant and by CIFAR.
K.C.\ is supported by a UBC Four Year Fellowship (6456).
M.E.D.\ acknowledges support from the Naval Research Laboratory by NASA under contract S-15633Y.
T.D.\ and M.T.L.\ are supported by an NSF Astronomy and Astrophysics Grant (AAG) award number 2009468.
E.C.F.\ is supported by NASA under award number 80GSFC24M0006.
G.E.F., S.C.S., and S.J.V.\ are supported by NSF award PHY-2011772.
K.A.G.\ and S.R.T.\ acknowledge support from an NSF CAREER award \#2146016.
A.D.J.\ and M.V.\ acknowledge support from the Caltech and Jet Propulsion Laboratory President's and Director's Research and Development Fund.
A.D.J.\ acknowledges support from the Sloan Foundation.
N.La.\ acknowledges the support from Larry W. Martin and Joyce B. O'Neill Endowed Fellowship in the College of Science at Oregon State University.
Part of this research was carried out at the Jet Propulsion Laboratory, California Institute of Technology, under a contract with the National Aeronautics and Space Administration (80NM0018D0004).
D.R.L.\ and M.A.M.\ are supported by NSF \#1458952.
M.A.M.\ is supported by NSF \#2009425.
C.M.F.M.\ was supported in part by the National Science Foundation under Grants No.\ NSF PHY-1748958 and AST-2106552.
A.Mi.\ is supported by the Deutsche Forschungsgemeinschaft under Germany's Excellence Strategy - EXC 2121 Quantum Universe - 390833306.
The Dunlap Institute is funded by an endowment established by the David Dunlap family and the University of Toronto.
P.N.\ acknowledges support from the BHI, funded by grants from the John Templeton Foundation and the Gordon and Betty Moore Foundation
K.D.O.\ was supported in part by NSF Grant No.\ 2207267.
T.T.P.\ acknowledges support from the Extragalactic Astrophysics Research Group at E\"{o}tv\"{o}s Lor\'{a}nd University, funded by the E\"{o}tv\"{o}s Lor\'{a}nd Research Network (ELKH), which was used during the development of this research.
H.A.R.\ is supported by NSF Partnerships for Research and Education in Physics (PREP) award No.\ 2216793.
S.M.R.\ and I.H.S.\ are CIFAR Fellows.
Portions of this work performed at NRL were supported by ONR 6.1 basic research funding.
J.D.R.\ also acknowledges support from start-up funds from Texas Tech University.
J.S.\ is supported by an NSF Astronomy and Astrophysics Postdoctoral Fellowship under award AST-2202388, and acknowledges previous support by the NSF under award 1847938.
C.U.\ acknowledges support from BGU (Kreitman fellowship), and the Council for Higher Education and Israel Academy of Sciences and Humanities (Excellence fellowship).
C.A.W.\ acknowledges support from CIERA, the Adler Planetarium, and the Brinson Foundation through a CIERA-Adler postdoctoral fellowship.
O.Y.\ is supported by the National Science Foundation Graduate Research Fellowship under Grant No.\ DGE-2139292.

==> authors_RevTeX.tex <==
\author{Gabriella Agazie}
\orcid{0000-0001-5134-3925}
\affiliation{Center for Gravitation, Cosmology and Astrophysics, Department of Physics, University of Wisconsin-Milwaukee,\\ P.O. Box 413, Milwaukee, WI 53201, USA}
\author{Jeremy G. Baier}
\orcid{0000-0002-4972-1525}
\affiliation{Department of Physics, Oregon State University, Corvallis, OR 97331, USA}
\author{Jerry Sun}
\affiliation{Department of Physics, Oregon State University, Corvallis, OR 97331, USA}
\author{Paul T. Baker}
\orcid{0000-0003-2745-753X}
\affiliation{Department of Physics and Astronomy, Widener University, One University Place, Chester, PA 19013, USA}
\author{Bence B\'{e}csy}
\orcid{0000-0003-0909-5563}
\affiliation{Department of Physics, Oregon State University, Corvallis, OR 97331, USA}
\author{Laura Blecha}
\orcid{0000-0002-2183-1087}
\affiliation{Physics Department, University of Florida, Gainesville, FL 32611, USA}
\author{Adam Brazier}
\orcid{0000-0001-6341-7178}
\affiliation{Cornell Center for Astrophysics and Planetary Science and Department of Astronomy, Cornell University, Ithaca, NY 14853, USA}
\affiliation{Cornell Center for Advanced Computing, Cornell University, Ithaca, NY 14853, USA}
\author{Paul R. Brook}
\orcid{0000-0003-3053-6538}
\affiliation{Institute for Gravitational Wave Astronomy and School of Physics and Astronomy, University of Birmingham, Edgbaston, Birmingham B15 2TT, UK}
\author{Sarah Burke-Spolaor}
\orcid{0000-0003-4052-7838}
\altaffiliation{Sloan Fellow}
\affiliation{Department of Physics and Astronomy, West Virginia University, P.O. Box 6315, Morgantown, WV 26506, USA}
\affiliation{Center for Gravitational Waves and Cosmology, West Virginia University, Chestnut Ridge Research Building, Morgantown, WV 26505, USA}
\author{Rand Burnette}
\orcid{0009-0008-3649-0618}
\affiliation{Department of Physics, Oregon State University, Corvallis, OR 97331, USA}
\author{J. Andrew Casey-Clyde}
\orcid{0000-0002-5557-4007}
\affiliation{Department of Physics, University of Connecticut, 196 Auditorium Road, U-3046, Storrs, CT 06269-3046, USA}
\author{Maria Charisi}
\orcid{0000-0003-3579-2522}
\affiliation{Department of Physics and Astronomy, Vanderbilt University, 2301 Vanderbilt Place, Nashville, TN 37235, USA}
\author{Shami Chatterjee}
\orcid{0000-0002-2878-1502}
\affiliation{Cornell Center for Astrophysics and Planetary Science and Department of Astronomy, Cornell University, Ithaca, NY 14853, USA}
\author{Tyler Cohen}
\orcid{0000-0001-7587-5483}
\affiliation{Department of Physics, New Mexico Institute of Mining and Technology, 801 Leroy Place, Socorro, NM 87801, USA}
\author{James M. Cordes}
\orcid{0000-0002-4049-1882}
\affiliation{Cornell Center for Astrophysics and Planetary Science and Department of Astronomy, Cornell University, Ithaca, NY 14853, USA}
\author{Neil J. Cornish}
\orcid{0000-0002-7435-0869}
\affiliation{Department of Physics, Montana State University, Bozeman, MT 59717, USA}
\author{Fronefield Crawford}
\orcid{0000-0002-2578-0360}
\affiliation{Department of Physics and Astronomy, Franklin \& Marshall College, P.O. Box 3003, Lancaster, PA 17604, USA}
\author{H. Thankful Cromartie}
\orcid{0000-0002-6039-692X}
\affiliation{National Research Council Research Associate, National Academy of Sciences, Washington, DC 20001, USA resident at Naval Research Laboratory, Washington, DC 20375, USA}
\author{Megan E. DeCesar}
\orcid{0000-0002-2185-1790}
\affiliation{George Mason University, Fairfax, VA 22030, resident at the U.S. Naval Research Laboratory, Washington, DC 20375, USA}
\author{Paul B. Demorest}
\orcid{0000-0002-6664-965X}
\affiliation{National Radio Astronomy Observatory, 1003 Lopezville Rd., Socorro, NM 87801, USA}
\author{Heling Deng}
\affiliation{Department of Physics, Oregon State University, Corvallis, OR 97331, USA}
\author{Lankeswar Dey}
\orcid{0000-0002-2554-0674}
\affiliation{Department of Physics and Astronomy, West Virginia University, P.O. Box 6315, Morgantown, WV 26506, USA}
\affiliation{Center for Gravitational Waves and Cosmology, West Virginia University, Chestnut Ridge Research Building, Morgantown, WV 26505, USA}
\author{Timothy Dolch}
\orcid{0000-0001-8885-6388}
\affiliation{Department of Physics, Hillsdale College, 33 E. College Street, Hillsdale, MI 49242, USA}
\affiliation{Eureka Scientific, 2452 Delmer Street, Suite 100, Oakland, CA 94602-3017, USA}
\author{Elizabeth C. Ferrara}
\orcid{0000-0001-7828-7708}
\affiliation{Department of Astronomy, University of Maryland, College Park, MD 20742, USA}
\affiliation{Center for Research and Exploration in Space Science and Technology, NASA/GSFC, Greenbelt, MD 20771}
\affiliation{NASA Goddard Space Flight Center, Greenbelt, MD 20771, USA}
\author{William Fiore}
\orcid{0000-0001-5645-5336}
\affiliation{Department of Physics and Astronomy, West Virginia University, P.O. Box 6315, Morgantown, WV 26506, USA}
\affiliation{Center for Gravitational Waves and Cosmology, West Virginia University, Chestnut Ridge Research Building, Morgantown, WV 26505, USA}
\author{Emmanuel Fonseca}
\orcid{0000-0001-8384-5049}
\affiliation{Department of Physics and Astronomy, West Virginia University, P.O. Box 6315, Morgantown, WV 26506, USA}
\affiliation{Center for Gravitational Waves and Cosmology, West Virginia University, Chestnut Ridge Research Building, Morgantown, WV 26505, USA}
\author{Gabriel E. Freedman}
\orcid{0000-0001-7624-4616}
\affiliation{Center for Gravitation, Cosmology and Astrophysics, Department of Physics, University of Wisconsin-Milwaukee,\\ P.O. Box 413, Milwaukee, WI 53201, USA}
\author{Emiko C. Gardiner}
\orcid{0000-0002-8857-613X}
\affiliation{Department of Astronomy, University of California, Berkeley, 501 Campbell Hall \#3411, Berkeley, CA 94720, USA}
\author{Kyle A. Gersbach}
\affiliation{Department of Physics and Astronomy, Vanderbilt University, 2301 Vanderbilt Place, Nashville, TN 37235, USA}
\author{Joseph Glaser}
\orcid{0000-0003-4090-9780}
\affiliation{Department of Physics and Astronomy, West Virginia University, P.O. Box 6315, Morgantown, WV 26506, USA}
\affiliation{Center for Gravitational Waves and Cosmology, West Virginia University, Chestnut Ridge Research Building, Morgantown, WV 26505, USA}
\author{Deborah C. Good}
\orcid{0000-0003-1884-348X}
\affiliation{Department of Physics and Astronomy, University of Montana, 32 Campus Drive, Missoula, MT 59812}
\author{Kayhan G\"{u}ltekin}
\orcid{0000-0002-1146-0198}
\affiliation{Department of Astronomy and Astrophysics, University of Michigan, Ann Arbor, MI 48109, USA}
\author{Jeffrey S. Hazboun}
\orcid{0000-0003-2742-3321}
\affiliation{Department of Physics, Oregon State University, Corvallis, OR 97331, USA}
\author{Ross J. Jennings}
\orcid{0000-0003-1082-2342}
\altaffiliation{NANOGrav Physics Frontiers Center Postdoctoral Fellow}
\affiliation{Department of Physics and Astronomy, West Virginia University, P.O. Box 6315, Morgantown, WV 26506, USA}
\affiliation{Center for Gravitational Waves and Cosmology, West Virginia University, Chestnut Ridge Research Building, Morgantown, WV 26505, USA}
\author{Aaron D. Johnson}
\orcid{0000-0002-7445-8423}
\affiliation{Center for Gravitation, Cosmology and Astrophysics, Department of Physics, University of Wisconsin-Milwaukee,\\ P.O. Box 413, Milwaukee, WI 53201, USA}
\affiliation{Division of Physics, Mathematics, and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}
\author{David L. Kaplan}
\orcid{0000-0001-6295-2881}
\affiliation{Center for Gravitation, Cosmology and Astrophysics, Department of Physics, University of Wisconsin-Milwaukee,\\ P.O. Box 413, Milwaukee, WI 53201, USA}
\author{Luke Zoltan Kelley}
\orcid{0000-0002-6625-6450}
\affiliation{Department of Astronomy, University of California, Berkeley, 501 Campbell Hall \#3411, Berkeley, CA 94720, USA}
\author{Joey S. Key}
\orcid{0000-0003-0123-7600}
\affiliation{University of Washington Bothell, 18115 Campus Way NE, Bothell, WA 98011, USA}
\author{Nima Laal}
\orcid{0000-0002-9197-7604}
\affiliation{Department of Physics, Oregon State University, Corvallis, OR 97331, USA}
\author{Michael T. Lam}
\orcid{0000-0003-0721-651X}
\affiliation{SETI Institute, 339 N Bernardo Ave Suite 200, Mountain View, CA 94043, USA}
\affiliation{School of Physics and Astronomy, Rochester Institute of Technology, Rochester, NY 14623, USA}
\affiliation{Laboratory for Multiwavelength Astrophysics, Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{William G. Lamb}
\orcid{0000-0003-1096-4156}
\affiliation{Department of Physics and Astronomy, Vanderbilt University, 2301 Vanderbilt Place, Nashville, TN 37235, USA}
\author{Bjorn Larsen}
\affiliation{Department of Physics, Yale University, New Haven, CT 06520, USA}
\author{T. Joseph W. Lazio}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Pasadena, CA 91109, USA}
\author{Natalia Lewandowska}
\orcid{0000-0003-0771-6581}
\affiliation{Department of Physics and Astronomy, State University of New York at Oswego, Oswego, NY 13126, USA}
\author{Tingting Liu}
\orcid{0000-0001-5766-4287}
\affiliation{Department of Physics and Astronomy, West Virginia University, P.O. Box 6315, Morgantown, WV 26506, USA}
\affiliation{Center for Gravitational Waves and Cosmology, West Virginia University, Chestnut Ridge Research Building, Morgantown, WV 26505, USA}
\author{Jing Luo}
\orcid{0000-0001-5373-5914}
\altaffiliation{Deceased}
\affiliation{Department of Astronomy \& Astrophysics, University of Toronto, 50 Saint George Street, Toronto, ON M5S 3H4, Canada}
\author{Ryan S. Lynch}
\orcid{0000-0001-5229-7430}
\affiliation{Green Bank Observatory, P.O. Box 2, Green Bank, WV 24944, USA}
\author{Chung-Pei Ma}
\orcid{0000-0002-4430-102X}
\affiliation{Department of Astronomy, University of California, Berkeley, 501 Campbell Hall \#3411, Berkeley, CA 94720, USA}
\affiliation{Department of Physics, University of California, Berkeley, CA 94720, USA}
\author{Dustin R. Madison}
\orcid{0000-0003-2285-0404}
\affiliation{Department of Physics, University of the Pacific, 3601 Pacific Avenue, Stockton, CA 95211, USA}
\author{Alexander McEwen}
\orcid{0000-0001-5481-7559}
\affiliation{Center for Gravitation, Cosmology and Astrophysics, Department of Physics, University of Wisconsin-Milwaukee,\\ P.O. Box 413, Milwaukee, WI 53201, USA}
\author{James W. McKee}
\orcid{0000-0002-2885-8485}
\affiliation{Department of Physics and Astronomy, Union College, Schenectady, NY 12308, USA}
\author{Maura A. McLaughlin}
\orcid{0000-0001-7697-7422}
\affiliation{Department of Physics and Astronomy, West Virginia University, P.O. Box 6315, Morgantown, WV 26506, USA}
\affiliation{Center for Gravitational Waves and Cosmology, West Virginia University, Chestnut Ridge Research Building, Morgantown, WV 26505, USA}
\author{Patrick M. Meyers}
\orcid{0000-0002-2689-0190}
\affiliation{Division of Physics, Mathematics, and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Chiara M. F. Mingarelli}
\orcid{0000-0002-4307-1322}
\affiliation{Department of Physics, Yale University, New Haven, CT 06520, USA}
\author{Andrea Mitridate}
\orcid{0000-0003-2898-5844}
\affiliation{Deutsches Elektronen-Synchrotron DESY, Notkestr. 85, 22607 Hamburg, Germany}
\author{David J. Nice}
\orcid{0000-0002-6709-2566}
\affiliation{Department of Physics, Lafayette College, Easton, PA 18042, USA}
\author{Stella Koch Ocker}
\orcid{0000-0002-4941-5333}
\affiliation{Division of Physics, Mathematics, and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}
\affiliation{The Observatories of the Carnegie Institution for Science, Pasadena, CA 91101, USA}
\author{Ken D. Olum}
\orcid{0000-0002-2027-3714}
\affiliation{Institute of Cosmology, Department of Physics and Astronomy, Tufts University, Medford, MA 02155, USA}
\author{Timothy T. Pennucci}
\orcid{0000-0001-5465-2889}
\affiliation{Institute of Physics and Astronomy, E\"{o}tv\"{o}s Lor\'{a}nd University, P\'{a}zm\'{a}ny P. s. 1/A, 1117 Budapest, Hungary}
\author{Polina Petrov}
\orcid{0000-0001-5681-4319}
\affiliation{Department of Physics and Astronomy, Vanderbilt University, 2301 Vanderbilt Place, Nashville, TN 37235, USA}
\author{Nihan S. Pol}
\orcid{0000-0002-8826-1285}
\affiliation{Department of Physics, Texas Tech University, Box 41051, Lubbock, TX 79409, USA}
\author{Henri A. Radovan}
\orcid{0000-0002-2074-4360}
\affiliation{Department of Physics, University of Puerto Rico, Mayag\"{u}ez, PR 00681, USA}
\author{Scott M. Ransom}
\orcid{0000-0001-5799-9714}
\affiliation{National Radio Astronomy Observatory, 520 Edgemont Road, Charlottesville, VA 22903, USA}
\author{Paul S. Ray}
\orcid{0000-0002-5297-5278}
\affiliation{Space Science Division, Naval Research Laboratory, Washington, DC 20375-5352, USA}
% \author{Joseph D. Romano}
% \orcid{0000-0003-4915-3246}
% \affiliation{Department of Physics, Texas Tech University, Box 41051, Lubbock, TX 79409, USA}
\author{Jessie C. Runnoe}
\orcid{0000-0001-8557-2822}
\affiliation{Department of Physics and Astronomy, Vanderbilt University, 2301 Vanderbilt Place, Nashville, TN 37235, USA}
\author{Alexander Saffer}
\orcid{0000-0001-7832-9066}
\altaffiliation{NANOGrav Physics Frontiers Center Postdoctoral Fellow}
\affiliation{National Radio Astronomy Observatory, 520 Edgemont Road, Charlottesville, VA 22903, USA}
\author{Shashwat C. Sardesai}
\orcid{0009-0006-5476-3603}
\affiliation{Center for Gravitation, Cosmology and Astrophysics, Department of Physics, University of Wisconsin-Milwaukee,\\ P.O. Box 413, Milwaukee, WI 53201, USA}
\author{Kai Schmitz}
\orcid{0000-0003-2807-6472}
\affiliation{Institute for Theoretical Physics, University of M\"{u}nster, 48149 M\"{u}nster, Germany}
\author{Xavier Siemens}
\orcid{0000-0002-7778-2990}
\affiliation{Department of Physics, Oregon State University, Corvallis, OR 97331, USA}
\affiliation{Center for Gravitation, Cosmology and Astrophysics, Department of Physics, University of Wisconsin-Milwaukee,\\ P.O. Box 413, Milwaukee, WI 53201, USA}
\author{Joseph Simon}
\orcid{0000-0003-1407-6607}
\altaffiliation{NSF Astronomy and Astrophysics Postdoctoral Fellow}
\affiliation{Department of Astrophysical and Planetary Sciences, University of Colorado, Boulder, CO 80309, USA}
\author{Magdalena S. Siwek}
\orcid{0000-0002-1530-9778}
\affiliation{Center for Astrophysics, Harvard University, 60 Garden St, Cambridge, MA 02138, USA}
\author{Sophia V. Sosa Fiscella}
\orcid{0000-0002-5176-2924}
\affiliation{School of Physics and Astronomy, Rochester Institute of Technology, Rochester, NY 14623, USA}
\affiliation{Laboratory for Multiwavelength Astrophysics, Rochester Institute of Technology, Rochester, NY 14623, USA}
\author{Ingrid H. Stairs}
\orcid{0000-0001-9784-8670}
\affiliation{Department of Physics and Astronomy, University of British Columbia, 6224 Agricultural Road, Vancouver, BC V6T 1Z1, Canada}
\author{Daniel R. Stinebring}
\orcid{0000-0002-1797-3277}
\affiliation{Department of Physics and Astronomy, Oberlin College, Oberlin, OH 44074, USA}
\author{Abhimanyu Susobhanan}
\orcid{0000-0002-2820-0931}
\affiliation{Max-Planck-Institut f\"{u}r Gravitationsphysik (Albert-Einstein-Institut), Callinstrasse 38, D-30167, Hannover, Germany}
\author{Joseph K. Swiggum}
\orcid{0000-0002-1075-3837}
\altaffiliation{NANOGrav Physics Frontiers Center Postdoctoral Fellow}
\affiliation{Department of Physics, Lafayette College, Easton, PA 18042, USA}
\author{Jacob Taylor}
\affiliation{Department of Physics, Oregon State University, Corvallis, OR 97331, USA}
\author{Stephen R. Taylor}
\orcid{0000-0003-0264-1453}
\affiliation{Department of Physics and Astronomy, Vanderbilt University, 2301 Vanderbilt Place, Nashville, TN 37235, USA}
\author{Jacob E. Turner}
\orcid{0000-0002-2451-7288}
\affiliation{Green Bank Observatory, P.O. Box 2, Green Bank, WV 24944, USA}
\author{Caner Unal}
\orcid{0000-0001-8800-0192}
\affiliation{Department of Physics, Middle East Technical University, 06531 Ankara, Turkey}
\affiliation{Department of Physics, Ben-Gurion University of the Negev, Be'er Sheva 84105, Israel}
\affiliation{Feza Gursey Institute, Bogazici University, Kandilli, 34684, Istanbul, Turkey}
\author{Michele Vallisneri}
\orcid{0000-0002-4162-0033}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Drive, Pasadena, CA 91109, USA}
\affiliation{Division of Physics, Mathematics, and Astronomy, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Rutger van~Haasteren}
\orcid{0000-0002-6428-2620}
\affiliation{Max-Planck-Institut f\"{u}r Gravitationsphysik (Albert-Einstein-Institut), Callinstrasse 38, D-30167, Hannover, Germany}
\author{Joris Verbiest}
\affiliation{Department of Physics, University of Central Florida, Orlando, FL 32816-2385, USA}
\author{Sarah J. Vigeland}
\orcid{0000-0003-4700-9072}
\affiliation{Center for Gravitation, Cosmology and Astrophysics, Department of Physics, University of Wisconsin-Milwaukee,\\ P.O. Box 413, Milwaukee, WI 53201, USA}
\author{Caitlin A. Witt}
\orcid{0000-0002-6020-9274}
\affiliation{Center for Interdisciplinary Exploration and Research in Astrophysics (CIERA), Northwestern University, Evanston, IL 60208, USA}
\affiliation{Adler Planetarium, 1300 S. DuSable Lake Shore Dr., Chicago, IL 60605, USA}
\author{David Wright}
\orcid{0000-0003-1562-4679}
\affiliation{Department of Physics, Oregon State University, Corvallis, OR 97331, USA}
\author{Olivia Young}
\orcid{0000-0002-0883-0688}
\affiliation{School of Physics and Astronomy, Rochester Institute of Technology, Rochester, NY 14623, USA}
\affiliation{Laboratory for Multiwavelength Astrophysics, Rochester Institute of Technology, Rochester, NY 14623, USA}

